Online A-Optimal Design and Active Linear Regression

We consider in this paper the problem of optimal experiment design where a decision maker can choose which points to sample to obtain an estimate $\hat{\beta}$ of the hidden parameter $\beta^{\star}$ of an underlying linear model. The key challenge of this work lies in the heteroscedasticity assumption that we make, meaning that each covariate has a different and unknown variance. The goal of the decision maker is then to figure out on the fly the optimal way to allocate the total budget of $T$ samples between covariates, as sampling several times a specific one will reduce the variance of the estimated model around it (but at the cost of a possible higher variance elsewhere). By trying to minimize the $\ell^2$-loss $\mathbb{E} [\lVert\hat{\beta}-\beta^{\star}\rVert^2]$ the decision maker is actually minimizing the trace of the covariance matrix of the problem, which corresponds then to online A-optimal design. Combining techniques from bandit and convex optimization we propose a new active sampling algorithm and we compare it with existing ones. We provide theoretical guarantees of this algorithm in different settings, including a $\mathcal{O}(T^{-2})$ regret bound in the case where the covariates form a basis of the feature space, generalizing and improving existing results. Numerical experiments validate our theoretical findings.

==> active.tex <==
\input{active/introduction}
\input{active/setting}
\input{active/appendix_concentration}
\input{active/naive}
\input{active/bandit}
\input{active/discussion}
\input{active/simulations}
\input{active/conclusion}

\setcounter{section}{0}
\renewcommand{\thesection}{\arabic{chapter}.\Alph{section}}

\input{active/appendix_proof_concentration}

\renewcommand{\thesection}{\arabic{chapter}.\arabic{section}}



==> def.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\hypersetup{
    colorlinks,
    linkcolor={red!80!black},
    citecolor={blue!60!black},
    urlcolor={blue!80!black}
}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}

%\usepackage[Algorithm]{algorithm}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{mathtools}
\usepackage[mathscr]{euscript}
\usepackage{xcolor}

\usepackage{natbib}
\usepackage{comment}

% images
\usepackage{epsfig}
\usepackage{float}
%\usepackage[justification=centering]{caption}
\usepackage{subcaption}
%\usepackage{subfig}
\usepackage{tikz, pgfplots}
\usepackage{wrapfig}

\newcommand{\bE}{\mathbb{E}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bX}{\mathbb{X}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\sL}{\mathscr{L}}

\newcommand{\eps}{\varepsilon}
\newcommand{\sig}{\sigma^2}

\newcommand{\Y}[1]{Y^{(#1)}}
\newcommand{\e}[1]{\eps^{(#1)}}
\newcommand{\Lr}{L_{\rho}}
\newcommand{\tX}{\tilde{\bX}}

\newcommand{\argmin}{\mbox{argmin}}
\newcommand{\argmax}{\mbox{argmax}}
\newcommand{\dist}{\mbox{dist}}
\newcommand{\Tr}{\mbox{Tr}}
\newcommand{\Sp}{\mbox{Sp}}
\newcommand{\et}{\quad\mbox{and}\quad}
\newcommand{\Gram}{\mbox{Gram}}
\newcommand{\iid}{i.i.d}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}
%\newcommand{\Com}{\mbox{Com}}
\def\eqsp{\;}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\dd}{\, \mathrm{d}}
\newcommand{\pinv}{^{-1}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\normLigne}[1]{\Vert#1\Vert}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
%\newcommand{\norm}[1]{\ensuremath{\Arrowvert #1 \Arrowvert}}
%\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\newcommand{\normd}[1]{\norm{#1}_2}
\newcommand{\normi}[1]{\norm{#1}_{\infty}}
\newcommand{\normpsi}[2]{\norm{#1}_{\psi_{#2}}}
\newcommand{\st}{^{\star}}
\newcommand{\bst}{\beta\st}
\newcommand{\pst}{p\st}
\newcommand{\bht}{\hat{\beta}}
\newcommand{\expe}[1]{\mathbb{E}\left[#1\right]}

\newcommand{\Dk}{\Delta^K}
\newcommand{\Dd}{\Delta^d}

\newcommand{\op}{\Omega(p)}
\newcommand{\ops}{\Omega(p\st)}
\newcommand{\hop}{\hat{\Omega}(p)}
\newcommand{\hsig}{\hat{\sigma}}
\newcommand{\usig}{\underline{\sigma}}
\newcommand{\osig}{\overline{\sigma}}
\newcommand{\hp}{\hat{p}}
\newcommand{\mud}{\mu^{(2)}}
\newcommand{\hmud}{\hat{\mu}^{(2)}}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\inv}{^{-1}}
\newcommand{\T}{^{\top}}
\newcommand{\XX}{X_k X_k^{\top}}
\newcommand{\skk}{\sum_{k=1}^K}
\newcommand{\skd}{\sum_{k=1}^d}
\newcommand{\sinn}{\sum_{i=1}^n}
\newcommand{\lm}{\lambda_{\min}}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cof}{Cof}
\DeclareMathOperator{\Com}{Com}
\newcommand{\fracm}[2]{\left. #1 \middle / #2 \right.}
\newcommand{\fraca}[2]{\left. #1 / #2 \right.}
\newcommand{\transpose}{^{\top}}

\allowdisplaybreaks
\setlength{\belowcaptionskip}{-0.9\baselineskip}


\newcommand{\bigo}{\mathcal{O}}
\newcommand{\bigot}{\widetilde{\mathcal{O}}}
\newcommand{\smallo}{{\scriptscriptstyle \mathcal{O}}}
\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\II}[1]{\mathbb{I}{\left\{#1\right\}}}
\newcommand{\dpart}[2]{\dfrac{\partial #1}{\partial #2}}

\newtheorem{assumption}{Assumption}
\newtheorem{cor}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
